Low-Power Low-Latency Keyword Spotting and Adaptive Control with a SpiNNaker 2 Prototype and Comparison with Loihi

We implemented two neural network based benchmark tasks on a prototype chip of the second-generation SpiNNaker (SpiNNaker 2) neuromorphic system: keyword spotting and adaptive robotic control. Keyword spotting is commonly used in smart speakers to listen for wake words, and adaptive control is used in robotic applications to adapt to unknown dynamics in an online fashion. We highlight the benefit of a multiply accumulate (MAC) array in the SpiNNaker 2 prototype which is ordinarily used in rate-based machine learning networks when employed in a neuromorphic, spiking context. In addition, the same benchmark tasks have been implemented on the Loihi neuromorphic chip, giving a side-by-side comparison regarding power consumption and computation time. While Loihi shows better efficiency when less complicated vector-matrix multiplication is involved, with the MAC array, the SpiNNaker 2 prototype shows better efficiency when high dimensional vector-matrix multiplication is involved.

==> Makefile <==

TEXMASTERFILE = synaptic_sampling.tex
BIBFILE       = synaptic_sampling.bib

MASTERFILEBASE = $(basename $(TEXMASTERFILE))

SOURCES        = $(TEXMASTERFILE) $(wildcard sections/*.tex)

pdf: $(SOURCES)
	echo $^
	-@sed -i -e 's/μ/\$$\\mu\$$/g' $(BIBFILE)
	-@pdflatex $(TEXMASTERFILE)
	-@bibtex   $(MASTERFILEBASE)
	-@pdflatex $(TEXMASTERFILE)
	-@pdflatex $(TEXMASTERFILE)

showpdf show:
	zathura $(MASTERFILEBASE).pdf >/dev/null 2>/dev/null &

clean:
	rm -f $(MASTERFILEBASE).acn $(MASTERFILEBASE).acr $(MASTERFILEBASE).alg $(MASTERFILEBASE).atoc \
		$(MASTERFILEBASE).aux $(MASTERFILEBASE).bbl $(MASTERFILEBASE).blg $(MASTERFILEBASE).glg \
		$(MASTERFILEBASE).gls $(MASTERFILEBASE).glsdefs $(MASTERFILEBASE).ist $(MASTERFILEBASE).loa \
		$(MASTERFILEBASE).lof $(MASTERFILEBASE).log $(MASTERFILEBASE).lol $(MASTERFILEBASE).lot \
		$(MASTERFILEBASE).nav $(MASTERFILEBASE).out $(MASTERFILEBASE).sbl $(MASTERFILEBASE).snm \
		$(MASTERFILEBASE).sym $(MASTERFILEBASE).toc $(MASTERFILEBASE).bcf $(MASTERFILEBASE).run.xml

